On the Power of Oblivious State Preparation

We put forth Oblivious State Preparation (OSP) as a cryptographic primitive that unifies techniques developed in the context of a quantum server interacting with a classical client. OSP allows a classical polynomial-time sender to input a choice of one out of two public observables, and a quantum polynomial-time receiver to recover an eigenstate of the corresponding observable -- while keeping the sender's choice hidden from any malicious receiver. We obtain the following results: - The existence of (plain) trapdoor claw-free functions implies OSP, and the existence of dual-mode trapdoor claw-free functions implies round-optimal (two-round) OSP. - OSP implies the existence of proofs of quantumness, test of a qubit, blind classical delegation of quantum computation, and classical verification of quantum computation. - Two-round OSP implies quantum money with classical communication, classically-verifiable position verification, and (additionally assuming classical FHE with log-depth decryption) quantum FHE. Several of these applications were previously only known via tailored LWE-based constructions, whereas our OSP-based constructions yield new results from a wider variety of assumptions, including hard problems on cryptographic group actions. Finally, towards understanding the minimal hardness assumptions required to realize OSP, we prove the following: - OSP implies oblivious transfer between one classical and one quantum party. - Two-round OSP implies public-key encryption with classical keys and ciphertexts. In particular, these results help to ''explain'' the use of public-key cryptography in the known approaches to establishing a ''classical leash'' on a quantum server. For example, combined with a result of Austrin et al. (CRYPTO 22), we conclude that perfectly-correct OSP cannot exist unconditionally in the (quantum) random oracle model.

==> two-round-OSP-alt.tex <==
\subsection{Two-round OSP from dual-mode TCFs}\label{subsec:OSP-dTCF}

\begin{theorem}
    Any dTCF satisfying \cref{def:dTCF} implies a two-round OSP.
\end{theorem}

\begin{proof}
    We will essentially adapt the amplification lemma for dTCFs shown in \cite[section 3.2]{10.1007/978-3-031-68382-4_8}. The construction is given in \cref{fig:two-round}, where $\delta = \delta(\secp)$ is the parameter from the lossy mode property of the dTCF.  

    \protocol{Two-round OSP from dTCF}{Two-round OSP from dTCF}{fig:two-round}{

        \begin{itemize}
            \item $S(1^\secp,b)$: Let $\ell = \secp/\delta$. For $i \in [\ell]$, sample $(\pparam_i,\sparam_i) \gets \Gen(1^\secp,b)$, and define $\msg_S \coloneqq (\pparam_1,\dots,\pparam_\ell)$ and $\state_S \coloneqq (\sparam_1,\dots,\sparam_\ell)$. 
            \item $R(\msg_S)$: Define $G : \{0,1\} \times \{0,1\}^{n \cdot \ell} \times \{0,1\}^{\ell-1} \to \{0,1\}^{m \cdot \ell}$ as \[G(c,x_1,\dots,x_\ell,r_1,\dots,r_{\ell-1}) = (y_1,\dots,y_\ell),\] where $r_\ell = c \oplus r_1 \oplus \dots \oplus r_{\ell-1}$, and $y_i = F_{\pparam_i,r_i}$ for each $i \in [\ell]$. Prepare the state \[\ket*{+} \otimes \ket*{\psi_{\pparam_1}} \otimes \dots \otimes \ket*{\psi_{\pparam_\ell}} \otimes \ket*{+}^{\otimes \ell-1},\] apply $G$ in superposition to a fresh register, and measure that register to obtain $(y_1,\dots,y_\ell)$. Next, measure all but the first qubit in the Hadamard basis to obtain $ d_1,\dots,d_\ell \in \{0,1\}^n, e_1,\dots,e_{\ell-1} \in \{0,1\}$. Set $\msg_R = (y_1,\dots,y_\ell,d_1,\dots,d_\ell,e_1,\dots,e_{\ell-1})$ and output the remaining qubit.
            
            \item $S_\out(\state_S,\msg_R)$: If $b = 0$, do the following.
            \begin{itemize}
                \item For $i \in [\ell]$, try running $\Invert(\sparam_i,0,y_i)$ and $\Invert(\sparam_i,1,y_i)$. If both or neither return $\bot$, then abort and output $\bot$. Otherwise, let $r_i$ be the bit for which inversion succeeded.
                \item Output $s = r_1 \oplus \dots \oplus r_\ell$.
            \end{itemize}
            Otherwise, if $b=1$, do the following.
            \begin{itemize}
                \item For $i \in [\ell]$, try running $\Invert(\sparam_i,0,y_i)$ and $\Invert(\sparam_i,1,y_i)$. If there does not exist an $i$ such that both return non-$\bot$, then abort and output $\bot$. Otherwise, let $i$ be an arbitrary index such that two preimages $x_{i,0},x_{i,1}$ were obtained.
                \item Output $s = d_{i} \cdot (x_{i,0} \oplus x_{i,1}) \oplus e_{i}$ (where we define $e_\ell = 0$).
            \end{itemize}
        \end{itemize}
    
    }

    We argue correctness separately for each $b \in \{0,1\}$. In the case $b = 0$, the properties of the dTCF imply that after measuring $(y_1,\dots,y_\ell)$, the receiver's state collapses to a state negligibly close to 
    \[\ket*{c} \otimes \ket*{x_1} \otimes \dots \otimes \ket*{x_\ell} \otimes \ket*{r_1} \otimes \dots \otimes \ket*{r_{\ell-1}}.\]
    Moreover, with all but negligible probability, $S_\out$ will not abort, and instead compute the correct choices of $r_1,\dots,r_{\ell-1}$, and $r_\ell = c \oplus r_1 \oplus \dots \oplus r_{\ell-1}$. In this case, $S_\out$ outputs $s = c$, ensuring correctness.

    In the case $b=1$, the properties of the dTCF imply that after measuring $(y_1,\dots,y_\ell)$, with probability at least $1-(1-\delta)^{\secp/\delta} > 1-\negl(\secp)$, there is some set $S \subseteq [\ell]$ of size at least 1 such that the following holds. The receiver's state collapses to a state negligibly close to a state that, for any $i \in S$, can be written as \[\frac{1}{\sqrt{2}}\ket*{0}\ket*{A + \Delta_0} + \frac{1}{\sqrt{2}}\ket*{1}\ket*{A + \Delta_1},\] where $A$ is a subspace of $\bbF_2^{n\ell + \ell - 1}$ of dimension $2^{|S|-1}$ and\footnote{Note that when $A$ is a subspace of size greater than 1, there are redundant ways to write the shifts $\Delta_0,\Delta_1$ and $\Delta_0 \oplus \Delta_1$, which is why we can provide a different definition for each choice of $i \in S$.} \[\Delta_0 \oplus \Delta_1 = (0^n,\dots,0^n,z_{i},0^n,\dots,0^n,0,\dots,0,f_{i},0,\dots,0).\] By a standard calculation, measuring all but the first qubit in the Hadamard basis yields a string $d \in \{0,1\}^{n\ell + \ell - 1}$ and a remaining state $Z^{d \cdot (\Delta_0 \oplus \Delta_1)}\ket*{+}.$ Moreover, with all but negligible probability, $S_\out$ will compute the correct $x_{i,0},x_{i,1}$ such that $x_{i,0} \oplus x_{i,1} = z_{i}$.  In this case, $S_\out$ outputs $s = d \cdot (\Delta_0 \oplus \Delta_1)$, thus ensuring correctness.
    
\end{proof}
